Towards Accurate Human Motion Prediction via Iterative Refinement

Human motion prediction aims to forecast an upcoming pose sequence given a past human motion trajectory. To address the problem, in this work we propose FreqMRN, a human motion prediction framework that takes into account both the kinematic structure of the human body and the temporal smoothness nature of motion. Specifically, FreqMRN first generates a fixed-size motion history summary using a motion attention module, which helps avoid inaccurate motion predictions due to excessively long motion inputs. Then, supervised by the proposed spatial-temporal-aware, velocity-aware and global-smoothness-aware losses, FreqMRN iteratively refines the predicted motion though the proposed motion refinement module, which converts motion representations back and forth between pose space and frequency space. We evaluate FreqMRN on several standard benchmark datasets, including Human3.6M, AMASS and 3DPW. Experimental results demonstrate that FreqMRN outperforms previous methods by large margins for both short-term and long-term predictions, while demonstrating superior robustness.

==> files/extra.tex <==
\begin{table*}[t]
\begin{center}
    \begin{tabular}{ |c | cccc| } 
    \hline
    dataset & \multicolumn{4}{c|}{Human3.6M} \\
    \hline
    milliseconds & 80ms & 400ms & 560ms & 1000ms  \\ 
    \hline
    LTD & 11.2 & 58.9 & 78.3 & 114.0\\
    \rowcolor{gray}
    HRI &  10.4 & 58.3 & 77.3 & 112.1 \\
    STDGCN & 10.6 & 57.9 & 76.3 & 109.7\\
    \rowcolor{gray}
    MMA & 10.2 & 57.3 & 75.9 & 110.1\\
    siMLPe & $\underline{9.6}$ & $\underline{57.3}$ & $\underline{75.7}$ & $\underline{109.4}$ \\ 
    \rowcolor{gray}
    \hline
    Ours & $\mathbf{9.1}$ & $\mathbf{55.5}$ & $\mathbf{74.5}$ & $\mathbf{109.2}$ \\ 
    \hline
\end{tabular}
\end{center}
\caption{Action-wise prediction results on Human3.6M dataset. MPJPE in millimeter at particular frames are reported. 256 samples are tested for each action. The best results are highlighted in \textbf{bold}, and the second best results are \underline{underlined}.} 
\label{tab:h36_both}
\end{table*}
%

%
\begin{table*}[t]\scriptsize
\begin{center}
\resizebox{\linewidth}{!}{
    \begin{tabular}{  |c | cccc | cccc | } 
      \hline
      dataset  & \multicolumn{4}{c|}{AMASS} & \multicolumn{4}{c|}{3DPW}  \\
      \hline
      milliseconds & 80ms & 400ms & 560ms & 1000ms & 80ms & 400ms & 560ms &  1000ms  \\ 
      \hline
      \rowcolor{gray}
      LTD & $\underline{10.3}$ & 44.6 &61.5& 91.2& $\underline{12.0}$ & 46.2& 59.1& 81.1\\ 
      HRI &  11.3 & 42.0& 51.7 &67.2& 12.6 & 45.4 &56.0 &73.7\\ 
      \rowcolor{gray}
      MMA & 11.0 & 41.2 & 50.7 & 65.8 & 12.4 & $\underline{44.4}$ & $\underline{54.7}$  & $\underline{71.8}$ \\
    siMLPe &  10.8&  $\underline{40.5}$ &$\underline{50.5}$ &$\underline{65.7}$& 12.1 & 44.5& 54.9  &72.2\\ 
    \rowcolor{gray}
      Ours  &  $\mathbf{9.8}$ &	$\mathbf{37.9}$&	$\mathbf{47.8}$&	$\mathbf{65.4}$& $\mathbf{11.6}$&	$\mathbf{42.8}$	&$\mathbf{53.3}$&	$\mathbf{71.0}$\\ 
      \hline
    \end{tabular}}
\end{center}
\caption{Short-term and long-term prediction results on AMASS and 3DPW datasets. The models are trained on the AMASS dataset. MPJPE in millimeter at particular frames are reported. The best results are highlighted in \textbf{bold}, and the second best results are \underline{underlined}.} 
\label{tab:amass_3dpw}
\end{table*}
%

\begin{table}[t]\scriptsize
\begin{center}
\resizebox{\linewidth}{!}{
    \begin{tabular}{ | c | cccc | } 
    \hline
      variant & 80ms & 400ms & 560ms &  1000ms \\ 
      \hline
     w/o reweighting & 9.4	&	56.2&	75.1&	109.4\\
     \rowcolor{gray}
     \hline
     \rowcolor{gray}
    ours & $\mathbf{9.1}$ & $\mathbf{55.5}$ & $\mathbf{74.5}$ & $\mathbf{109.2}$	 \\ 
     \hline
    \end{tabular}}
\end{center}
\caption{Ablation on loss configurations.} 
\label{tab:abla_aug_loss}
\end{table}


\begin{table}[t]
	\centering
	\begin{tabular}{|c|l|}
		\hline
		$x_t$  &  $t^{th}$-level noised latent \\
		$\alpha_t$ & $1 - \beta_t$, $\beta_t$: forward process variance \\
		\hline
	\end{tabular}
	%}
\end{table}

\begin{table}[t]
	\centering
	\begin{tabular}{|c|l|}
		\hline
		$\bar{\alpha}_t$    & $\prod_{s=1}^{t} \alpha_s$ \\ 
		$\epsilon_0$  &  standard Gaussian \\
		\hline
	\end{tabular}
	%}
\end{table}

\begin{table}[t]
	\centering
	\begin{tabular}{|c|c|}
		\hline
            \multicolumn{2}{|c|}{concept mapping} \\
            \hline
		past motion $\mathcal{D}$  & $c$  \\
		future motion $\mathcal{X}^0$ & $x_0$ \\
		  $\mathcal{X}^k$ & $x_t$ \\ 
    $N$ & number of generated samples \\ 
		\hline
  
	\end{tabular}
	%}
\end{table}

$\begin{aligned} L_r(\phi)=  \min _i \|\hat{\mathcal{X}}_i-\mathcal{X} \|^2+  \sum_{i=1}^N \|\hat{\mathcal{X}}_i-\mathcal{Y}_i \|^2 +\gamma \frac{1}{N(N-1)} \sum_{i=1}^N \sum_{j \neq i}^N \exp  (-\frac{d^2 (\hat{\mathcal{X}}_i, \hat{\mathcal{X}}_j )}{\sigma} )\end{aligned}$


$$\epsilon_t = \epsilon_\theta(x_t, f_\phi(c), t), x_0 = $$
$$z_0 = z_\theta(z_t, f_\phi(c), t)$$

$x_{t-1} =\frac{1}{\sqrt{\alpha_t}}\left(x_t-\frac{\beta_t}{\sqrt{1-\bar{\alpha}_t}} \epsilon_t\right)+\sqrt{\beta_t} \epsilon_0$

% $z_{t-1} =\Tilde{\mu}(z_{t-1})+\sqrt{\beta_t} \epsilon_0, x_0 = g_\lambda(z_0)$

$$x_0 = G_{\theta}(x_t, c, t)$$

$$x_{t-1} = \Tilde{\mu}(x_{t-1})+\sqrt{\beta_t} \epsilon_0$$

\begin{equation}
\label{eq::reverse_diff}
    p_{\theta}(x_{t-1}|x_t)=\mathcal{N}(x_{t-1}; \textcolor{red}{\mu_{\theta}(x_t, t)},\sigma_{\theta}^2(x_t, t)\textrm{I}).
\end{equation}

\begin{equation}
\label{eq::reverse_diff}
    p_{\theta}(x_{t-1}|x_t, c)=\mathcal{N}(x_{t-1}; \mu_{\theta}(x_t, \textcolor{red}{c}, t),\sigma_{\theta}^2(x_t,\textcolor{red}{c}, t)\textrm{I}).
\end{equation}

$$\hat{\mathcal{X}}$$

\begin{table}[t]
	\centering
	\begin{tabular}{|c|l|}
		\hline
		$c$ & $y^{1:H}$: clean past motion \\
            $\Tilde{x}_0$ & $\Tilde{x}_0^{1:F}$: initial future motion reconstruction \\
		\hline
	\end{tabular}
	%}
\end{table}

\begin{table}[t]
	\centering
	\begin{tabular}{|c|l|}
		\hline
		$x_t$  & $x_t^{1:F}$: $t^{th}$-level noised future motion \\
		$\Tilde{x}_0$ & $\Tilde{x}_0^{1:F}$: initial future motion reconstruction \\
            $\mathrm{PE}$ & positional encoding \\
		\hline
	\end{tabular}
	%}
\end{table}

\begin{table}[t]
	\centering
	\begin{tabular}{|c|l|}
		\hline
		$x_0^{j}$  & future motion of $j^{th}$ joint\\
            $y^j$  & motion history of $j^{th}$ joint \\
		\hline
	\end{tabular}
	%}
\end{table}

$$\Tilde{x}_0 = F(x_t, t)$$

$$\hat{x}_0 \leftarrow [\hat{y}; \hat{x}_0] = R(y, \Tilde{x}_0)$$

$$\hat{x}_0 \leftarrow [\hat{y}; \hat{x}_0] = R(y, F(x_t, t)) \coloneqq G_{\theta}(y_t, x, t)$$

$$
\|(y^j-\hat{y}^j) \cdot \lambda^j\|_1 + \|(x_0^j-\hat{x}_0^j) \cdot \lambda^j\|_1
$$

$$\|(x^j-\hat{x}^j) \cdot \lambda^j\|_2$$

$$G_{\theta}(x_t, c, t) = $$


    $$\hat{x}_0 \leftarrow [\hat{y}; \hat{x}_0] = R(y, F(x_t, t)) \coloneqq G_{\theta}(x_t, c, t)$$

$L(\theta):=\mathbb{E}_{x_t, t}[\|\epsilon-\epsilon_\theta(x_t, c, t)\|^2]$

$$\bm{x_t=\sqrt{\bar{\alpha}_t} x_0+\sqrt{1-\bar{\alpha}_t} \epsilon_0}$$

$$q(x_{t-1} | x_t, x_0)$$

$$p_{\theta}(x_{t-1} | x_t, \textcolor{red}{c})$$

$$L(\theta):=\mathbb{E}_{x_t, t}[\|\epsilon_0-\epsilon_\theta(x_t, \textcolor{red}{c}, t)\|^2]$$


    $$\hat{x}_0 \leftarrow [\hat{y}; \hat{x}_0] = R(y, F(x_t, t)) \coloneqq G_{\theta}(x_t, c, t)$$
    
\begin{table*}[t]
\begin{center}
\begin{tabular}{c c | c c c c c c c c}
\hline 
 &  & \multicolumn{7}{c}{Human3.6M} \\
\hline
Method &  Type & APD $\uparrow$ & APDE $\downarrow$ & ADE $\downarrow$ & FDE $\downarrow$ & MMADE $\downarrow$ & MMFDE $\downarrow$ & CMD $\downarrow$ & FID $\downarrow$ \\
\rowcolor{gray}
\hline 
DLow [1] & Div. & 11.741 & 3.781 & 0.425 & 0.518 & 0.495 & 0.531 & 4.927 & 1.255 \\
GSPS [2] & Div. & 14.757 & 6.749 & 0.389 & 0.496 & 0.476 & 0.525 & 10.758 & 2.103 \\
\rowcolor{gray}
DivSamp [3] & Div. & \textbf{15.310} & 7.479 & 0.370 & 0.485 & 0.475 & 0.516 & 11.692 & 2.083  \\
\hline
BeLFusion [4] & Fid. & 7.602 & 1.662 & 0.372 & 0.474 & \textbf{0.473} & 0.507 & 5.988 & 0.209 \\
\hline
\hline
\rowcolor{gray}
Ours & Fid. & 7.753 & \textbf{1.570} & \textbf{0.351} & \textbf{0.458} & 0.495 & \textbf{0.507} & \textbf{3.279} & \textbf{0.106} \\
\hline
\end{tabular}
\end{center}
\end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{c c | c c c c c c c}
\hline 
&  & \multicolumn{6}{c}{ AMASS } \\
\hline 
Method &  Type & APD $\uparrow$ & APDE $\downarrow$ & ADE $\downarrow$ & FDE $\downarrow$ & MMADE $\downarrow$ & MMFDE $\downarrow$ & CMD $\downarrow$  \\
\rowcolor{gray}
\hline 
DLow [1] & Div. & 13.170 & 4.243 & 0.590 & 0.612 & 0.618 & 0.617 & 15.185 \\
GSPS [2] & Div. & 12.465 & 4.678 & 0.563 & 0.613 & 0.609 & 0.633 & 18.404 \\
\rowcolor{gray}
DivSamp [3] & Div. & \textbf{24.724} & 15.837 & 0.564 & 0.647 & 0.623 & 0.667 & 50.239  \\
\hline
BeLFusion [4] & Fid. & 9.376 & \textbf{1.977} & 0.513 & 0.560 & 0.569 & 0.585 & 16.995 \\
\hline
\hline
\rowcolor{gray}
Ours & Fid. & 10.320 & 2.117 & \textbf{0.490} & \textbf{0.543} & \textbf{0.467} & \textbf{0.465} & \textbf{10.502} \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{lrrrrr}
\toprule
Model (Macro-AUC $\uparrow$) &  \textsc{Wiki} &  \textsc{Reddit}  & \textsc{ML-Rating} & \textsc{ML-Genre}  \\
\midrule
GCNII [1] & $\underline{67.45 \pm 1.61}$ & $61.13 \pm 1.37$ & $\underline{71.45 \pm 3.74}$ & $\underline{62.12 \pm 1.18} \\
\midrule
DySAT [2] & $54.27 \pm 4.27$ & $\underline{66.51 \pm 0.30}$ & $53.89 \pm 5.83$ & $51.89 \pm 1.77$ \\
EvolveGCN [3] & $58.92 \pm 2.10$ & $62.22 \pm 1.60$ & $61.31 \pm 2.47$ & $51.13 \pm 2.47$ \\
Ours & $\mathbf{69.17 \pm 1.84}$ & $\mathbf{66.70 \pm 1.59}$ & $\mathbf{73.72 \pm 0.23}$ & $\mathbf{75.04 \pm 1.51}$ \\
\bottomrule
\end{tabular}
\label{tab:results_auc_new}
\end{table*}

\begin{table}[t]
	\centering
	\begin{tabular}{|c|l|}
		\hline
		$f_{\psi}$    & motion history encoder \\ 
		$\epsilon_{\theta}$  &  noise predictor \\
            $r_{\phi}$  &  motion refiner \\
		\hline
	\end{tabular}
	%}
\end{table}

\begin{table}[t]
	\centering
	\begin{tabular}{|c|l|}
		\hline
		$x_t$  &  $t^{th}$-level noised latent \\
		$\epsilon_0$ & standard Gaussian \\
            $\mu_q$ & forward process posterior mean \\
		\hline
	\end{tabular}
	%}
\end{table}
\begin{table}[t]
	\centering
	\begin{tabular}{|c|l|}
		\hline
		$y$  & motion history \\
		$\hat{y}$ & reconstructed motion history \\
            $\hat{x}$ & generated motion future  \\
            $\mathrm{DCT}$ & discrete cosine transform \\
		\hline
	\end{tabular}
	%}
\end{table}

\begin{table}[t]
	\centering
	\begin{tabular}{|c|l|}
		\hline
		$v_t$  & node of interest at snapshot $t$\\
		$w_t, u_t$ & structural one-hop neighbors of $v_t$\\
            $v_{t+1}, v_{t-1}$ & temporal one-hop neighbors of $v_t$ \\
		\hline
	\end{tabular}
	%}
\end{table}

\begin{table}[t]
	\centering
	\begin{tabular}{|c|l|}
		\hline
		$\vc_l$  & $l^{th}$ kinematic chain of one pose\\
            $b_l^{i}$  & bone length of the $i^{th}$ bone on $\vc_l$ \\
            $l(\vc_l)$  & total number of bones of $\vc_l$ \\
		\hline
	\end{tabular}
	%}
\end{table}

Specifically, let $\mX = \{\vx_{1}, \vx_{2}, \ldots, \vx_{F}\}$ denotes predicted motion, where $\vx \in \sR^{J\times 3}$ describes the 3D coordinates of one particular human pose. 
Based on the kinematic structure of the human body, each pose $\vx$ can be described by $\mathcal{L}$ kinematic chains.
Let $\vc_l$ denote the $l^{th}$ kinematic chain, $b_l^{i}$ denote the bone length of the $i^{th}$ bone on $\vc_l$, and $l(\vc_l)$ denote the total number of bones of $\vc_l$.
Form the spatial perspective, suppose that the $j^{th}$ joint is the $j'^{th}$ joint on chain $\vc_l$.
We define:
%
\begin{equation}
\label{eq::lambda_s}
\lambda_j^f \propto \frac{j'}{l(\vc_l)}\ln\left(\sum_{i'=1}^{j'}b_l^{i'}\right).
\end{equation}
%

\begin{table*}[t]
\centering
\begin{tabular}{lrrrrr}
\toprule
Model (Macro-AUC $\uparrow$) &  \textsc{Wiki} &  \textsc{Reddit}  & \textsc{ML-Rating} & \textsc{ML-Genre}  \\
\midrule
DySAT [1] & $54.27 \pm 4.27$ & $66.51 \pm 0.30$ & $53.89 \pm 5.83$ & $51.89 \pm 1.77$ \\
EvolveGCN [2] & $58.92 \pm 2.10$ & $62.22 \pm 1.60$ & $61.31 \pm 2.47$ & $51.13 \pm 2.47$ \\
Ours & $\mathbf{69.17 \pm 1.84}$ & $\mathbf{66.70 \pm 1.59}$ & $\mathbf{73.72 \pm 0.23}$ & $\mathbf{75.04 \pm 1.51}$ \\
\bottomrule
\end{tabular}
\label{tab:results_auc_new}
\end{table*}

\begin{table*}\scriptsize
\centering
\begin{tabular}{cccc}
\toprule
Model Type & Space Complexity & Time Complexity & Sequential Ops. \\
\midrule
DySAT [1] & $O(LET+LF^2+LTNF+LNT^2)$ & $O(LETF+LTNF^2+LNT^2F)$ & $O(1)$\\
EvolveGCN [2] & $O(ET+LTF^2+LTNF)$  & $O(LETF+LTNF^2)$ & $O(T)$\\
\midrule
Ours & $O(ET+LF^2+LTNF)$ & $O(LETF+LTNF^2)$ & $O(1)$ \\
\bottomrule
\end{tabular}
\label{tab:complexity}
\end{table*}

\begin{table}[t]
	\centering
	\begin{tabular}{|c|l|}
		\hline
		$L$  & number of layers \\ 
		$N$  & number of nodes per snapshot \\
            $T$  & number of snapshots \\
            $E$  & number of edges per snapshot \\
            $F$  & feature dimension \\
		\hline
	\end{tabular}
	%}
\end{table}

\begin{table*}[t]
\centering
\begin{tabular}{c c | c c c c c}
\hline 
&  & \multicolumn{5}{c}{ Human3.6M } \\
\hline 
Method &  Type & APD $\uparrow$ & ADE $\downarrow$ & FDE $\downarrow$ & MMADE $\downarrow$ & MMFDE $\downarrow$ \\
\hline 
\rowcolor{gray}
STARS [1] & Div. &  \textbf{15.884} & 0.358 & \textbf{0.445} & \textbf{0.442} & \textbf{0.471} \\
MotionDiff [2] & Div. & 15.353 & 0.411 & 0.509 & 0.508 & 0.536 \\
\hline
\rowcolor{gray}
Ours & Fid. & 7.753 & \textbf{0.351} & \textbf{0.458} & \textbf{0.495} & \textbf{0.507} \\
\hline
\end{tabular}
\end{table*}

%
\begin{table*}[t]\scriptsize
\begin{center}
\resizebox{\linewidth}{!}{
    \begin{tabular}{  |c | cccc|cccc | cccc|cccc | } 
      \hline
      dataset  & \multicolumn{8}{c|}{AMASS} & \multicolumn{8}{c|}{3DPW}  \\
      \hline
      milliseconds & 80ms & 160ms & 320ms & 400ms & 560ms & 720ms & 880ms & 1000ms & 80ms & 160ms & 320ms & 400ms & 560ms & 720ms & 880ms & 1000ms  \\ 
      \hline
      \rowcolor{gray}
      convSeq2Seq & 20.6 &36.9 &59.7 &67.6& 79.0& 87.0 &91.5 &93.5 &18.8 &32.9& 52.0 &58.8 &69.4& 77.0 &83.6 &87.8 \\ 
      LTD-10-10 & $\underline{10.3}$& $\underline{19.3}$ &36.6& 44.6 &61.5& 75.9 &86.2& 91.2& $\underline{12.0}$ & $\underline{22.0}$ &38.9 &46.2& 59.1& 69.1 &76.5& 81.1\\ 
      \rowcolor{gray}
      LTD-10-25 & 11.0 &20.7 &37.8 &45.3 &57.2 &65.7& 71.3& 75.2 &12.6 &23.2& 39.7 &46.6 &57.9& 65.8 &71.5& 75.5\\
      HRI \cite{DBLP:conf/eccv/MaoLS20} &  11.3 &20.7 &35.7& 42.0& 51.7 &58.6 &63.4 &67.2& 12.6 &23.1 &39.0& 45.4 &56.0 &63.6& 69.7 &73.7\\ 
      \rowcolor{gray}
      MMA  & 11.0 & 20.3 & 35.0 & 41.2 & 50.7 & 57.4 & $\underline{61.9}$ & 65.8 & 12.4 & 22.6 & 38.1 & $\underline{44.4}$ & $\underline{54.7}$ & $\underline{62.1}$ & $\underline{67.9}$ & $\underline{71.8}$ \\
    siMLPe &  10.8& 19.6 &$\underline{34.3}$& $\underline{40.5}$ &$\underline{50.5}$& $\underline{57.3}$& 62.4 &$\underline{65.7}$& 12.1 &22.1 &$\underline{38.1}$& 44.5& 54.9 &62.4& 68.2 &72.2\\ 
    \rowcolor{gray}
      Ours  &  $\mathbf{9.8}$ &	$\mathbf{17.8}$&	$\mathbf{31.8}$&	$\mathbf{37.9}$&	$\mathbf{47.8}$&	$\mathbf{55.3}$&	$\mathbf{60.7}$&	$\mathbf{65.4}$& $\mathbf{11.6}$	&$\mathbf{20.8}$&	$\mathbf{36.4}$&	$\mathbf{42.8}$	&$\mathbf{53.3}$&	$\mathbf{61.0}$&	$\mathbf{66.9}$&	$\mathbf{71.0}$\\ 
      \hline
    \end{tabular}}
\end{center}
\caption{Short-term and long-term prediction results on AMASS and 3DPW datasets. The models are trained on the AMASS dataset. MPJPE in millimeter at particular frames are reported. The best results are highlighted in \textbf{bold}, and the second best results are \underline{underlined}.} 
\label{tab:amass_3dpw}
\end{table*}


\begin{table*}[t]\scriptsize
\begin{center}
\resizebox{\linewidth}{!}{
    \begin{tabular}{ |c |cccc| cccc | cccc| cccc| } 
    \hline
    scenarios  & \multicolumn{4}{c|}{walking} & \multicolumn{4}{c|}{eating} & \multicolumn{4}{c|}{smoking} & \multicolumn{4}{c|}{discussion} \\
    \hline
    milliseconds & 80ms & 400ms & 560ms & 1000ms & 80ms & 400ms & 560ms & 1000ms & 80ms & 400ms & 560ms & 1000ms & 80ms & 400ms & 560ms & 1000ms  \\ 
    \hline
    \rowcolor{gray} 
    ResSup \cite{DBLP:conf/cvpr/MartinezB017} & 23.2 & 66.1 & 71.6 & 79.1 & 16.8 & 61.7 & 74.9 & 98.0 & 18.9 & 65.4 & 78.1 & 102.1 & 25.7 & 91.3 & 109.5 & 131.8  \\ 
    convSeq2Seq \cite{DBLP:conf/cvpr/LiZLL18} & 17.7 & 63.6 & 72.2 & 82.3 & 11.0 & 48.4 & 61.3 & 87.1 & 11.6 & 48.9 & 60.0 & 81.7 & 17.1 & 77.6 & 98.1 & 129.3 \\ 
    \rowcolor{gray}
    LTD-50-25 \cite{DBLP:conf/iccv/MaoLSL19} & 12.3 & 44.4 & 50.7 & 60.3 & 7.8 & 38.6 & 51.5 & 75.8 & 8.2 & 39.5 & 50.5 & 72.1 & 11.9 & 68.1 & 88.9 & 118.5 \\
    LTD-10-10 \cite{DBLP:conf/iccv/MaoLSL19} & 11.1 & 42.9 & 53.1 & 70.7 & 7.0 & 37.3 & 51.1 & 78.6 & 7.5 & 37.5 & 49.4 & 71.8 & 10.8 & 65.8 & 88.1 & 121.6 \\
    \rowcolor{gray}
    HRI \cite{DBLP:conf/eccv/MaoLS20} & 10.0 & 39.8 & 47.4 & 58.1 & 6.4 & 36.2 & 50.0 & 75.7 & 7.0 & 36.4 & 47.6 & 69.5 & 10.2 & 65.4 & 86.6 & 119.8\\
    STDGCN \cite{DBLP:conf/cvpr/MaNLZL22} & 11.2 & 42.8 & 49.6 & 58.9 & 6.5 & 36.8 & 50.0 & 74.9 & 7.3 & 37.5 & 48.8 & 69.9 & 10.2 & 64.4 & 86.1 & $\underline{116.9}$\\
    \rowcolor{gray}
    MMA  \cite{DBLP:journals/ijcv/MaoLSL21} & 9.9 & $\underline{39.0}$ & $\underline{46.2}$ & 57.1 & 6.2 & $\underline{35.3}$ & $\underline{48.6}$ & $\underline{73.7}$ & 6.8 & $\underline{35.5}$ & $\underline{46.5}$ & $\mathbf{68.7}$ & 9.9 & $\underline{64.0}$ & $\underline{85.2}$ & 117.5 \\
    siMLPe \cite{DBLP:conf/wacv/GuoDSLAM23} & $\underline{9.9}$ & 39.6 & 46.8 & $\underline{55.7}$ & $\underline{5.9}$ & 36.1 & 49.6 & 74.5 & $\underline{6.5}$ & 36.3 & 47.2 & 69.3 & $\underline{9.4}$ & 64.3 & 85.7 & $\mathbf{116.3}$\\
    \rowcolor{gray}
    \hline
    Ours & $\mathbf{9.0}$ & $\mathbf{36.7}$ & $\mathbf{44.5}$ & $\mathbf{54.1}$ & $\mathbf{5.6}$ & $\mathbf{33.9}$ & $\mathbf{47.2}$ & $\mathbf{73.1}$ & $\mathbf{6.2}$ & $\mathbf{35.1}$ & $\mathbf{46.9}$ & $\underline{69.2}$ & $\mathbf{8.7}$ & $\mathbf{62.9}$ & $\mathbf{84.7}$ & 117.1 \\ 
    \hline
    scenarios  & \multicolumn{4}{c|}{directions} & \multicolumn{4}{c|}{greeting} & \multicolumn{4}{c|}{phoning} & \multicolumn{4}{c|}{posing} \\
    \hline
    milliseconds & 80ms & 400ms & 560ms & 1000ms & 80ms & 400ms & 560ms & 1000ms & 80ms & 400ms & 560ms & 1000ms & 80ms & 400ms & 560ms & 1000ms  \\ 
    \hline
    \rowcolor{gray}
    ResSup \cite{DBLP:conf/cvpr/MartinezB017}& 21.6 & 84.1 & 101.1 & 129.1 & 31.2 & 108.8 & 126.1 & 153.9 & 21.1 & 76.4 & 94.0 & 126.4 & 29.3 & 114.3 & 140.3 & 183.2 \\ 
    convSeq2Seq \cite{DBLP:conf/cvpr/LiZLL18}& 13.5 & 69.7 & 86.6 & 115.8 & 22.0 & 96.0 & 116.9 & 147.3 & 13.5 & 59.9 & 77.1 & 114.0 & 16.9 & 92.9 & 122.5 & 187.4 \\ 
    \rowcolor{gray}
    LTD-50-25 \cite{DBLP:conf/iccv/MaoLSL19} & 8.8 & 58.0 & 74.2 & 105.5 & 16.2 & 82.6 & 104.8 & 136.8 & 9.8 & 50.8 & 68.8 & 105.1 & 12.2 & 79.9 & 110.2 & 174.8\\
    LTD-10-10 \cite{DBLP:conf/iccv/MaoLSL19} & 8.0 & 54.9 & 76.1 & 108.8 & 14.8 & 79.7 & 104.3 & 140.2 & 9.3 & 49.7 & 68.7 & 105.1 & 10.9 & 75.9 & 109.9 & 171.7\\
    \rowcolor{gray}
    HRI  \cite{DBLP:conf/eccv/MaoLS20}& 7.4 & 56.5 & 73.9 & 106.5 & 13.7 & 78.1 & 101.9 & 138.8 & 8.6 & 49.2 & 67.4 & 105.0 & 10.2 & 75.8 & 107.6 & 178.2\\ 
    STDGCN \cite{DBLP:conf/cvpr/MaNLZL22} & 7.5 & 56.0 & 73.3 & 105.9 & 14.0 & 77.3 & 100.2 & $\mathbf{136.4}$ & 8.7 & 48.8 & 66.5 & $\mathbf{102.7}$ & 10.2 & $\underline{73.3}$ & $\underline{102.8}$ & $\underline{167.0}$\\
    \rowcolor{gray}
    MMA  \cite{DBLP:journals/ijcv/MaoLSL21}& 7.2 & $\underline{55.0}$ & $\underline{72.4}$ & $\underline{105.7}$ & 13.6 & $\underline{77.2}$ & 100.5 & 136.7 & 8.4 & $\underline{48.4}$ & 66.5 & 104.6 & 9.8 & 74.9 & 105.8 & 172.9\\
    siMLPe \cite{DBLP:conf/wacv/GuoDSLAM23} & $\underline{6.5}$ & 55.8 & 73.1 & 106.7 & $\underline{12.4}$ & 77.3 & $\underline{99.8}$ & 137.5 & $\underline{8.1}$ & 48.6 & $\underline{66.3}$ & 103.3 & $\underline{8.8}$ & 73.8 & 103.4 & 168.7\\
    \rowcolor{gray}
    \hline
    Ours & $\mathbf{6.3}$ & $\mathbf{52.8}$ & $\mathbf{69.8}$ & $\mathbf{104.4}$ & $\mathbf{11.6}$ & $\mathbf{72.8}$ & $\mathbf{97.7}$ & $\underline{136.5}$ & $\mathbf{7.6}$ & $\mathbf{46.5}$ & $\mathbf{64.6}$ & $\underline{103.3}$ & $\mathbf{8.3}$ & $\mathbf{70.7}$ & $\mathbf{101.0}$ & $\mathbf{166.4}$\\ 
    \rowcolor{gray}
    \hline
    scenarios  & \multicolumn{4}{c|}{purchases} & \multicolumn{4}{c|}{sitting} & \multicolumn{4}{c|}{sitting down} & \multicolumn{4}{c|}{taking photo} \\
    \hline
    milliseconds & 80ms & 400ms & 560ms & 1000ms & 80ms & 400ms & 560ms & 1000ms & 80ms & 400ms & 560ms & 1000ms & 80ms & 400ms & 560ms & 1000ms  \\ 
    \hline
    \rowcolor{gray}
    ResSup \cite{DBLP:conf/cvpr/MartinezB017}& 28.7 & 100.7 & 122.1 & 154.0 & 23.8 & 91.2 & 113.7 & 152.6 & 31.7 & 112.0 & 138.8 & 187.4 & 21.9 & 87.6 & 110.6 & 153.9 \\
    convSeq2Seq \cite{DBLP:conf/cvpr/LiZLL18}& 20.3 & 89.9 & 111.3 & 151.5 & 13.5 & 63.1 & 82.4 & 120.7 & 20.7 & 82.7 & 106.5 & 150.3 & 12.7 & 63.6 & 84.4 & 128.1 \\ 
    \rowcolor{gray}
    LTD-50-25 \cite{DBLP:conf/iccv/MaoLSL19} & 15.2 & 78.1 & 99.2 & 134.9 & 10.4 & 58.3 & 79.2 & 118.7 & 17.1 & 76.4 & 100.2 & 143.8 & 9.6 & 54.3 & 75.3 & 118.8\\
    LTD-10-10 \cite{DBLP:conf/iccv/MaoLSL19} & 13.9 & 75.9 & 99.4 & 135.9 & 9.8 & 55.9 & 78.5 &  118.8 & 15.6 & 71.7 & 96.2 & 142.2 & 8.9 & 51.7 & 72.5 & 116.3\\
    \rowcolor{gray}
    HRI \cite{DBLP:conf/eccv/MaoLS20} & 13.0 & 73.9 & 95.6 & 134.2 & 9.3 & 56.0 & 76.4 & 115.9 & 14.9 & 72.0 & 97.0 & 143.6 & 8.3 & 51.5 & 72.1 & 115.9\\ 
    STDGCN \cite{DBLP:conf/cvpr/MaNLZL22} & 13.2 & 74.0 & 95.7 & $\mathbf{132.1}$ & 9.1 & $\underline{54.6}$ & $\underline{75.1}$ & 114.8 & 14.7 & $\mathbf{70.0}$ & $\mathbf{94.4}$ & $\mathbf{139.0}$ & 8.2 & $\underline{50.2}$ & $\underline{70.5}$ & 112.9\\
    \rowcolor{gray} 
    MMA  \cite{DBLP:journals/ijcv/MaoLSL21} & 12.8 & 72.8 & 94.5 & 133.1 & 9.1 & 55.4 & 75.8 & 115.0 & 14.7 & 71.3 & 96.0 & 141.8 & 8.2 & 51.1 & 71.8 & 115.2\\
    siMLPe \cite{DBLP:conf/wacv/GuoDSLAM23} & $\underline{11.7}$ & $\underline{72.4}$ & $\underline{93.8}$ & $\underline{132.5}$ & $\underline{8.6}$ & 55.2 & 75.4 & $\mathbf{114.1}$ & $\underline{13.6}$ & 70.8 & 95.7 & 142.4 & $\underline{7.8}$ & 50.8 & 71.0 & $\underline{112.8}$\\
    \rowcolor{gray}
    \hline
    Ours & $\mathbf{11.1}$ & $\mathbf{71.7}$ & $\mathbf{93.0}$ & 132.7 & $\mathbf{8.4}$ & $\mathbf{53.8}$ & $\mathbf{74.7}$ & $\underline{114.5}$ & $\mathbf{13.5}$ & $\underline{70.4}$ & $\underline{95.1}$ & $\underline{141.6}$ & $\mathbf{7.5}$ & $\mathbf{49.1}$ & $\mathbf{69.5}$ & $\mathbf{111.6}$\\ 
    \hline
    scenarios  & \multicolumn{4}{c|}{waiting} & \multicolumn{4}{c|}{walking dog} & \multicolumn{4}{c|}{walking together} & \multicolumn{4}{c|}{average} \\
    \hline
    milliseconds & 80ms & 400ms & 560ms & 1000ms & 80ms & 400ms & 560ms & 1000ms & 80ms & 400ms & 560ms & 1000ms & 80ms & 400ms & 560ms & 1000ms  \\ 
    \hline
    \rowcolor{gray}
    ResSup \cite{DBLP:conf/cvpr/MartinezB017}& 23.8 & 87.7 & 105.4 & 135.4 & 36.4 & 110.6 & 128.7 & 164.5 & 20.4 & 67.3 & 80.2 & 98.2 & 25.0 & 88.3 & 106.3 & 136.6  \\ 
    convSeq2Seq \cite{DBLP:conf/cvpr/LiZLL18}& 14.6 & 68.7 & 87.3 & 117.7 & 27.7 & 103.3 & 122.4 & 162.4 & 15.3 & 61.2 & 72.0 & 87.4 & 16.6 & 72.7 & 90.7 & 124.2\\ 
    \rowcolor{gray}
    LTD-50-25 \cite{DBLP:conf/iccv/MaoLSL19} & 10.4 & 59.2 & 77.2 & 108.3 & 22.8 & 88.7 & 107.8 & 156.4 & 10.3 & 46.3 & 56.0 & 65.7 & 12.2 & 61.5 & 79.6 & 112.4\\
    LTD-10-10 \cite{DBLP:conf/iccv/MaoLSL19} & 9.2 & 54.4 & 73.4 & 107.5 & 20.9 & 86.6 & 109.7 & 150.1 & 9.6 & 44.0 & 55.7 & 69.8 & 11.2 & 58.9 & 78.3 & 114.0\\
    \rowcolor{gray}
    HRI \cite{DBLP:conf/eccv/MaoLS20} & 8.7 & 54.9 & 74.5 & 108.2 & 20.1 & 86.3 & 108.2 & 146.9 & 8.9 & 41.9 & 52.7 & 64.9 & 10.4 & 58.3 & 77.3 & 112.1 \\
    STDGCN \cite{DBLP:conf/cvpr/MaNLZL22} & 8.7 & 53.6 & 71.6 & $\underline{103.7}$ & 20.4 & 84.6 & 105.7 & 145.9 & 8.9 & 43.8 & 54.4 & 64.6 & 10.6 & 57.9 & 76.3 & 109.7\\
    \rowcolor{gray}
    MMA  \cite{DBLP:journals/ijcv/MaoLSL21} & 8.4 & 53.8 & 72.7 & 105.1 & 19.6 & $\underline{84.1}$ & $\mathbf{105.1}$ & $\underline{141.4}$ & 8.5 & $\underline{41.1}$ & 51.2 & 63.2 & 10.2 & 57.3 & 75.9 & 110.1\\
    siMLPe \cite{DBLP:conf/wacv/GuoDSLAM23}& $\underline{7.8}$ & $\underline{53.2}$ & $\underline{71.6}$ & 104.6 & $\underline{18.2}$ & $\mathbf{83.6}$ & $\underline{105.6}$ & $\mathbf{141.2}$ & $\underline{8.4}$ & 41.2 & $\underline{50.8}$ & $\mathbf{61.5}$ & $\underline{9.6}$ & $\underline{57.3}$ & $\underline{75.7}$ & $\underline{109.4}$ \\ 
    \rowcolor{gray}
    \hline
    Ours & $\mathbf{7.2}$ & $\mathbf{50.5}$ & $\mathbf{69.0}$ & $\mathbf{103.4}$ & $\mathbf{17.8}$ & 87.0 & 112.0 & 147.5 & $\mathbf{7.7}$ & $\mathbf{38.5}$ & $\mathbf{48.5}$ & $\underline{61.9}$ & $\mathbf{9.1}$ & $\mathbf{55.5}$ & $\mathbf{74.5}$ & $\mathbf{109.2}$ \\ 
    \hline
\end{tabular}}
\end{center}
\caption{Action-wise prediction results on Human3.6M dataset. MPJPE in millimeter at particular frames are reported. 256 samples are tested for each action. The best results are highlighted in \textbf{bold}, and the second best results are \underline{underlined}.} 
\label{tab:h36_both}
\end{table*}
